On an Information and Control Architecture for Future Electric Energy Systems

This paper presents considerations towards an information and control architecture for future electric energy systems driven by massive changes resulting from the societal goals of decarbonization and electrification. This paper describes the new requirements and challenges of an extended information and control architecture that need to be addressed for continued reliable delivery of electricity. It identifies several new actionable information and control loops, along with their spatial and temporal scales of operation, which can together meet the needs of future grids and enable deep decarbonization of the electricity sector. The present architecture of electric power grids designed in a different era is thereby extensible to allow the incorporation of increased renewables and other emerging electric loads.

==> Sec/Notes.tex <==
\begin{figure}
    \centering
    \includegraphics[width = \linewidth]{Fig/Layered_arch.png}
    \caption{A layered architecture of the electric grid \copyright Joule 2021}
    \label{fig:layered_arch}
\end{figure}



the architecture of today's electric energy system. 



Challenges that arise from the societal objective of decarbonization. The decarbonization has 

The new technological features of the electric grid allow for partial solution to the challenges above. However, many more research and innovation would be needed. A particular piece of the research innovation would be on how to lay out a proper architecture for the evoltuion of the electric grid. 

Here we take a design philosophy of addressing the decision making to be made at local level as much as possible, but not any further. We draw a contrast with a fully distributed architecture or a fully integrated architecture. 



Challenges from carbon-neutral transition

The interplay between reliability, affordability, and sustainability. 

Opportunities might arise from the tighter coupling of multiple energy resources, 
also from tapping into the flexible demands
also from grid-forming inverters
also from advanced AI and data sciences decision tools. 

The ultimate envelop of success will likely to be achieved by a combination of hardware investment and cyber investment. This paper is outlining a possible cyber infrastructure that would align the resources and hardware in a most efficient and innovation-compatible manner. 

We draw upon past experiences in the Internet, computer architecture, as well as control system architecture. We argue that a proper design of architecture would be conducibe to many system-level innovations. 



\textbf{New features of the grid}
\begin{itemize}
    \item Intelligent edge
    \item Low-inertia grid
    \item Potentially new roles of aggregators, due to DER and EV in distribution systems
    \item Massive, multiple-domain information in the grid
    \begin{itemize}
        \item Massive, multiple-domain data, such as PMU, load data, weather data, market data
        \item Data privacy and security
    \end{itemize}
    \item Transportation electrification
\end{itemize}

\noindent \textbf{Overarching Goal:} Reliability, (Market) Efficiency, and Environmental Responsibility


\textcolor{blue}{Anupam: This philosophy should be clarified. While more choices should be available to customers thereby turning them into prosumers; wider information sharing would be beneficial for coordinated (gas + electric + transportation) regional planning. this would mean we need improved modeling and also co-simulation software}



\textcolor{blue}{(1) long duration energy storage: with retirement of 'base-load' coal power in favor of intermittent renewables there is a probability that renewable generation may be insufficient for multiple hours. Thus there is a need for research into long duration energy storage that can provide backup cite [https://www.energy.gov/eere/long-duration-storage-shot]}

\textcolor{blue}{
(2) improved forecasting and scenario analysis tools: granular and accurate forecasting of DER resources such as rooftop PVs will be needed to manage the distribution operations
\cite{homer2020electric}
}

\textcolor{blue}{
(3) power system planning: system planning can't be focused around peak load since the load patterns could shift, and uncertainty and variability will increase
}




\subsection{Distribution System Planning} \label{sec:IRP}
Today typically the Distribution Company (DISCO) owns the distribution grid and is responsible for planning and operations to maintain its reliability. It is responsible for procuring power to supply the demand of all its customers. Some DISCOs generate their own power (particularly in the vertically integrated paradigm), or purchase power from other entities via power purchase agreements, or from a wholesale electricity market. 

Utilities undertake a comprehensive process to develop Integrated Resource Plans (IRPs) to ensure that there is an adequate portfolio of supply-side and demand-side resources to meet the peak demand and energy needs of their customers at least cost, typically over a 10-20 year planning horizon \cite{wilson2013best}. Resource planning requirements differ from state to state. The plans account for variety of risks including load growth, fuel prices, fuel diversity and emissions, and require the involvement of state public utility commissions (PUCs) along with other stakeholders. Thus societal choices are introduced into the planning of the grid infrastructure, for example, through state renewable portfolio standards.

\subsection{Distribution System Operations} \label{sec:dist_ops}

Many DISCOs are using Supervisory Control and Data Acquisition (SCADA) systems for ensuring the correct operation of substation equipment, through data acquisition, monitoring and control of the distribution system. SCADA combines hardware, software and communications to monitor various equipment, send control signals and perform key operations such as voltage control, load balancing, power quality monitoring, fault protection etc.
The first layer in this is the hardware that actuates and monitors the system conditions, including reclosers, capacitor controls, voltage regulators, fault current indicators etc. The second layer does the data collection, communication and control through remote terminal units (RTUs) and intelligent electronic devices (IEDs). The third layer is responsible for communications with the host platform typically in the control center. The fourth layer is the software platform that integrates the multiple data streams, analyses it and provides the capabilities for display and interaction to the human operators.

Today most intelligence at the distribution level is in substations with limited control and visibility downstream through devices such as reclosers, customer smart meters etc. In the future more intelligence is likely to be deployed behind the customer meters via EV software, smart thermostats, home stationary batteries etc.

\subsection{Transmission System Planning} \label{sec:trans_planning}

Transmission systems in the US are planned on a regional basis with the aim being to meet future demand and maintain grid reliability as the fleet of generating resources and their locations continues to evolve. In some areas Regional Transmission Organizations (RTOs) conduct the transmission planning process. Transmission owners are predominantly compensated for their investments in the transmission network via cost-based rates.


\subsection{Transmission System Operations} \label{sec:trans_ops}
The Independent System Operator (ISO) is responsible for running the wholesale market into which GENCOs and DISCOs submit their offers and bids for power.
The ISO also has a number of other functions needed for the reliable operation of the transmission level grid, including administering products for energy, ancillary services, capacity and financial transmission rights. ISOs also coordinate with the Transmission Companies (TRANSCOs) on transmission system maintenance and planning.

In non-ISO areas the vertically integrated electric companies continue to be responsible for both transmission and distribution system operations.

% Future of distribution system:
%Historically the direction of electricity was uni-directional from the sub-station to the mains of the customer. This has begun to change in recent years with rooftop solar PV installations being able to inject their power to the distribution system. 

%

\subsection{Incorporating DERs into Wholesale Markets} \label{sec:ferc2222}
% FERC 2222 and DER aggregators role.

In 2020 the Federal Energy Regulatory Commission (FERC) issued Order 2222 to allow aggregations of distributed energy resources (DERs) to participate in wholesale electricity markets \cite{ferc2222}. This will allow DERs to provide energy, ancillary services and capacity to compete in wholesale markets with large-scale generators. This order permits Aggregators to pool multiple small DERs so as to meet minimum size thresholds and other requirements of the ISOs. The current participation models, market software and other mechanisms will need to be modified in order to account for the suite of technologies that might be included in DERs, including electric storage, distributed generation, demand response, energy efficiency, thermal storage and electric vehicles. Currently only two ISOs in the US namely New York (NYISO) and California (CAISO) have DER aggregation programs.

Currently ISOs do not have visibility into the distribution grid, but this could be a concern when large numbers of DERs start participating in the wholesale market via a Aggregators. While the DER Aggregator will try to maximize its profit in the wholesale markets it will have an impact to the operation of the distribution grid. It is important to ensure that the participation of DERs in the wholesale market does not violate any of the distribution system constraints. Thus, there is a need for a coordination framework to exchange information and control signals between the Aggregator, the DISCO and the ISO. 

Researchers are looking into the question of whether there is a need for Distribution System Operators (DSOs) to coordinate retail transactions and operations, analogous to the way ISOs coordinate these at the wholesale level. A distribution level market may be able to account for distribution constraints and provide appropriate price signals through distributed locational marginal prices (dLMPs) \cite{haider2020toward}.



%%%%%%%%%%%%%%%%%%%%%%%
\subsection{IBR Control} \label{sec:IBRctrl}
The DC energy resources, e.g., wind/solar farms, and energy storage, interface with an AC power grid via inverters. These DC resources are termed inverter-based resources (IBRs). Figure \ref{fig:grid_connected_inverter} shows a DC energy resource connect to a microgrid at a point of common coupling (PCC) via an inverter and a low-pass filter. The inverter is regulated by a feedback controller that observes the inverter terminal voltage and current and tunes the inverter modulation index, in order to track a setpoint given. There are two types of inverter control schemes: the grid-following control, and the grid-forming control. The inverter with the grid-following (grid-forming) controller is called the grid-following (grid-forming) inverter. 
\begin{figure}[htb]
    \centering
    \includegraphics[width = \linewidth]{Fig/InverterControl.png}
    \caption{A grid-connected inverter with a controller}
    \label{fig:grid_connected_inverter}
\end{figure}
\subsubsection{Conventional Grid-following control} The grid-following inverter is designed for the situation where the frequency and voltage magnitude at the PCC are in a nominal range, and it cannot regulate the frequency and voltage magnitude in a power grid. As a result, the grid-following inverter alone cannot form an autonomous power grid. The setpoints for the grid-following controller are real and reactive power which can be determined by solving the optimal power flow (OPF) problem \cite{6805674,6417004,SU201245}. A phase lock loop (PLL), a current controller, and a Pulse Width Modulation (PWM) module are three typical functional blocks in a grid-following controller \cite{9528341}. Note that almost all grid-connected inverters are grid-following inverters in modern power systems. %[\textbf{Discussing existing research works on the grid-following}] 

\subsubsection{New Grid-forming control} The grid-forming inverter can regulate the terminal voltage magnitude and frequency at the PCC by tracking the frequency and voltage setpoints, and it can provide  restoration support\cite{9528341,lin2020research}. The setpoints of a grid-forming controller are frequency and voltage magnitude. The grid-forming controllers can be broken down into three categories \cite{lin2020research}: 1) droop controllers \cite{4118327}, 2) synchronverter controllers \cite{beck2007virtual,5456209}, and 3) virtual oscillator controllers \cite{7317584}. The \underline{droop controllers} stabilize grid frequencies (voltage magnitudes) by changing real (reactive) power that DGs inject to the grid \cite{195899,4118327}, and they can also determine how much real and reactive power that each DG contributes in order to eliminate real and reactive power imbalance. A droop controller typically consists of a power controller, a voltage controller, current controller, and a PWM module \cite{9528341,4118327}. A \underline{synchronverter controller} enables an inverter to mimic the behavior of a synchronous machine \cite{beck2007virtual,5456209}. Such a control strategy is motivated by the fact that the contemporary grid apparatus, e.g., protection and control, is designed for a grid where synchronous generators are dominated. Engineering an inverter-based resource that behaves like a synchronous generator makes it easier to be integrated into an existing power grid, since its host grid does not need to have many changes. Another attractive feature of the synchronverters is that it can provide their host power grid with inertia, which makes the grid less sensitive to disturbances. A \underline{virtual oscillator controller} is programmed such that the controlled inverter can mimic a limit-cycle oscillator that can be synchronized with other inverters without communication. The parameter tuning procedure of a virtual oscillator controller can achieved in a systematical way without heavily relying on time-domain simulations \cite{7317584}.





\subsection{Cyber-Physical Security} \label{sec:cps}
The decision making in operation of bulk power systems heavily relies on massive distributed measurements. For example, the electricity market operation is built upon a wide-area state estimator that takes SCADA data as inputs. The automatic generation control (AGC) changes the setpoints of generators based on the SCADA measurements that may be thousands miles away from the control center where the AGC is located. Due to such a tight coupling between measurements and operational decisions, there arises a concern that a malicious adversary may compromise the grid operation by manipulating the distributed, poorly-secured sensors. For example, Xie \emph{et al.} \cite{xie2011integrity} envision a scenario where an attacker can be benefited financially by deliberately tampering the SCADA measurements. Reference \cite{8345676} suggests that the grid can be destabilized by an attacker who intrudes into the frequency/tie-line flow measurements of the AGC system. A substantial body of literature is devoted to address the cyber-physical security of power grids \cite{song2018intelligent,9167203, mohan2020comprehensive, dibaji2019systems}. 

Next we present one possible way that can secure the distributed measurements of AGC from cyber attacks. Figure \ref{fig:AGC} shows a simplified scheme of the AGC in modern power systems. The AGC essentially is a feedback loop which takes as inputs frequency $\omega$ and tie-line flow $P_{\text{tie}}$, and tunes the setpiont $P_{\text{set}}$ of each generator under controlled. The distributed measurements $P_{\text{tie}}$ and $\omega$ might not be well-secured. Suppose that measurements  $\omega$ and $P_ {\text{tie}}$ are maliciously manipulated, then the setpoints $P_{\text{tie}}$ computed by the AGC are wrong. As a result, the grid security is compromised. To detect the cyber attacks, reference \cite{8345676} proposes a watermarking-based approach. The following introduces the basic idea of the watermarking approach. A private, small signal, i.e., the watermark, is superposed upon the actual setpoint. The watermark has certain statistical signature that can be reflected in the distribution measurements. By examining if the statistical signature exist in the tie-line flows and frequency, a wide class of cyber attacks can be detected with rigorous performance guarantee \cite{8345676}. 
\begin{figure}
    \centering
    \includegraphics[width = 3.5in]{Fig/AGC_Attack.png}
    \caption{A dynamic-watermarking approach to securing the AGC of a bulk transmission system. ACE: area control error. SACE: smoothed ACE. PI: proportional-integral. GTG: governor turbine generator. (Source: Fig. 2 of reference \cite{8345676} \copyright IEEE 2018)}
    \label{fig:AGC}
\end{figure}




\subsection{Energy Storage Coordination}
Battery energy storage (BES) can play a part of providing grid operation services, such as frequency regulation, and peak shaving. All ISOs and RTOs have established a pay-for-performance regulation market where BES participants can obtain financial rewards by providing charging and discharging response in a timely manner \cite{8383984}. A wide body of research is devoted to address the BES's participation in the regulation market. For example, strategies of using BES for grid frequency regulation is proposed in \cite{8383984,5109519,8935195,zecchino2021optimal}. Reference \cite{9449728} investigates the impact of battery degradation on the BES participation in the regulation market. Reference \cite{8027056} proposes a scheme that leverages BES for both peak shaving and frequency regulation.
Next, we take the scheme reported reference \cite{8383984} as an illustrative example. In a pay-for-performance market, the ISO can issue regulation signals $r[k] \in [-1, 1]$ to all BES participants at time $k$. Each BES participant has freedom to choose dispatch power $b[k]$ at time $k$ as well as the BES capacity $C$ that participants in the market. Define $\mathbf{b}:= \{b[1],b[2], \ldots, b[K]\}$ and $\mathbf{r}:= \{r[1],r[2], \ldots, r[K]\}$. Given a market period $k\in\{1, 2, \ldots,K\}$, a BES participant is rewarded based on a performance function $\rho\left(C, \mathbf{b}, \mathbf{r} \right)$ that quantifies how well its BES tracks the regulation signal $r[k]$ \cite{8383984}. Since there is limited regulation capacity that is needed for the grid operation, the regulation market may become saturated. As a result, naive strategies of choosing $C$ and $b[k]$ might render the BES services hardly profitable \cite{8383984} for the BES participants. To address such a challenge facing the BES participants, the optimal BES participation problem can be formulated as follows \cite{8383984}:
\begin{subequations} \label{eq:BESS_coordination}
    \begin{align}
        \min_{C, b[k] \forall k}\quad & \rho\left(C, \mathbf{b}, \mathbf{r} \right) \pi C - A\left(\mathbf{b}\right)\\
        \text{s.t.}\quad & \rho\left(C, \mathbf{b}, \mathbf{r}\right)-\underline{\rho} \ge 0,\\
        & 0\le C \le \bar{C},\\
        & -\bar{b}\le b[k] \le \bar{b}, \quad \forall{k}\\
        & \underline{e} \le e[k] \le \bar{e}, \quad \forall{k}\\
        & 
        \begin{aligned}
        e[k] &- e[k-1] = \Delta K \gamma \texttt{ReLU}(b[k])\\ &- \Delta K \texttt{ReLU}(-b[k])/\gamma \quad \forall{k} \label{eq:SOC_dyn}
        \end{aligned}
    \end{align} 
\end{subequations}
where $A(\cdot)$ is the battery aging cost function \cite{8383984}; $\underline{\rho}$ is the minimal performance index specified by the ISO; $\bar{C}$ is the maximal battery capacity; $\bar{b}$ is the BES power rating; $\underline{e}$ and $\bar{e}$ denote the battery upper and lower MWh limits; $ e[k]$ is the BES state of charge (SOC) at time $k$; $\Delta K$ and $\gamma$ are the length of a dispatch interval, and charging and discharging efficiency coefficient, respectively; and $\texttt{ReLU}(\cdot)$ is the Rectified Linear Unit. Constraint \eqref{eq:SOC_dyn} defines the SOC dynamics. Due to the unavailability of the future regulation signal $\mathbf{r}$, optimization \eqref{eq:BESS_coordination} cannot be solved. To address such an issue, reference \cite{8383984} re-formulates the optimal battery participation as a chance-constrained optimization problem \cite{8383984}.

%%%%%%%%%%%%%%%%%%%
%% Section II
Before  embarking  on  what  are  the  future  challenges,  we begin by describing the current architecture of power systems.To  understand  it,  requires  an  understanding  of  the  decomposition  along  temporal  and  spatial  scales.  It  also  requires an understanding of the entities involved in transmission and distribution, and the planning and operational aspects involved.Finally, it is important to understand how all this is achieved by a collection of control loops, and how they are organized. 

%% II A:
The Temporal and Spatial Scales:
The temporal scales are broadly as follows:
1)  At the slowest time-scale, the physical grid infrastructure is planned based on a time horizon of years or decades.This  is  where  decisions  on  building  new  plants  or transmission lines are made.
2)  The  commitment  and  dispatch  of  resources  via  whole-sale market mechanisms is done on the daily to hourly scale.  Some  generators  require  on  the  order  of  hours to  start-up  or  shut  down.  Hence  the  “unit  commitment problem,” that is the schedule for the availability of different generators, is typically done one day in advance. Also,  generators  submit  their  bids  on  an  hour-by-hour basis for the next day, and the System Operator decides on  which  bids  to  accept  based  on  estimated  demand,lowest  cost,  and  to  ensure  reliability.  Further,  on the given day, generators are economically dispatched on a
5-minute  (typically)  basis,  so  that  the  System  Operator can balance generation and supply.
3)  Finally, stability, i.e., regulating frequency at 60 Hz (in the US, and 50 Hz elsewhere), and voltage, is addressed by control loops in the seconds to milliseconds scale.


Next, we take the scheme reported in \cite{8383984} as an illustrative example. In a pay-for-performance market, the ISO can issue regulation signals $r[k] \in [-1, 1]$ to all BES participants at time $k$. Each BES participant has freedom to choose dispatch power $b[k]$ at time $k$ as well as the BES capacity $C$ that participants in the market. Define $\mathbf{b}:= \{b[1],b[2], \ldots, b[K]\}$ and $\mathbf{r}:= \{r[1],r[2], \ldots, r[K]\}$. Given a market period $k\in\{1, 2, \ldots,K\}$, a BES participant is rewarded based on a performance function $\rho\left(C, \mathbf{b}, \mathbf{r} \right)$ that quantifies how well its BES tracks the regulation signal $r[k]$ \cite{8383984}. Since there is limited regulation capacity that is needed for the grid operation, the regulation market may become saturated. As a result, naive strategies of choosing $C$ and $b[k]$ might render the BES services hardly profitable \cite{8383984} for the BES participants. To address such a challenge facing the BES participants, the optimal BES participation problem can be formulated as follows \cite{8383984}:
\begin{subequations} \label{eq:BESS_coordination}
    \begin{align}
        \min_{C, b[k] \forall k}\quad & \rho\left(C, \mathbf{b}, \mathbf{r} \right) \pi C - A\left(\mathbf{b}\right)\\
        \text{s.t.}\quad & \rho\left(C, \mathbf{b}, \mathbf{r}\right)-\underline{\rho} \ge 0,\\
        & 0\le C \le \bar{C},\\
        & -\bar{b}\le b[k] \le \bar{b}, \quad \forall{k}\\
        & \underline{e} \le e[k] \le \bar{e}, \quad \forall{k}\\
        & 
        \begin{aligned}
        e[k] &- e[k-1] = \Delta K \gamma \texttt{ReLU}(b[k])\\ &- \Delta K \texttt{ReLU}(-b[k])/\gamma \quad \forall{k} \label{eq:SOC_dyn}
        \end{aligned}
    \end{align} 
\end{subequations}
where $A(\cdot)$ is the battery aging cost function \cite{8383984}; $\underline{\rho}$ is the minimal performance index specified by the ISO; $\bar{C}$ is the maximal battery capacity; $\bar{b}$ is the BES power rating; $\underline{e}$ and $\bar{e}$ denote the battery upper and lower MWh limits; $ e[k]$ is the BES state of charge (SOC) at time $k$; $\Delta K$ and $\gamma$ are the length of a dispatch interval, and charging and discharging efficiency coefficient, respectively; and $\texttt{ReLU}(\cdot)$ is the Rectified Linear Unit. Constraint \eqref{eq:SOC_dyn} defines the SOC dynamics. Due to the unavailability of the future regulation signal $\mathbf{r}$, optimization \eqref{eq:BESS_coordination} cannot be solved. To address such an issue, reference \cite{8383984} re-formulates the optimal battery participation as a chance-constrained optimization problem \cite{8383984}.


%%%%%%%%%%%%%%%%%%%

\begin{table*}[t]
	\caption{Existing Control Loops in Modern Power Systems}
	\label{tab:ExistingLoops}
	\centering

	\begin{tabular}{c|l|l|p{0.3\textwidth}}
	\hline

	\hline
	\textbf{Loop \#} & \textbf{Pair of Entities} & \textbf{Interaction} & \textbf{Control Actions (timescale)}\\
	\hline
		 1 & GENCO - Gas pipeline/marketer & Fuel supply & \begin{itemize}
		 \item Fuel reliability (real-time)
		 \item Gas purchases (day-ahead to months-ahead)
		 \end{itemize}\\
		 \hline
		 2 & GENCO - ISO & Power balance & 
        \begin{itemize}
		     \item AGC (sec/min)
		     \item Economic Dispatch (hours)
		     \item Unit Commitment (days-ahead)
		 \end{itemize}\\
		 \cline{3-4}
		 & & Capacity scheduling & Outage coordination (weeks/months)\\
		\cline{3-4}
        & & Capacity planning & Generation planning (years)\\
	\hline
	3 & ISO - TRANSCO & Transmission reliability & 
	\begin{itemize}
		     \item Monitoring voltage, flows, line limits etc. (real-time)
		     \item Outage coordination (weeks/months)
		     \item Transmission line planning (years)
		 \end{itemize}\\
		 \hline
	4 & GENCO & Generator control & 
		     AVR and Governor actions (sec)
		     \\
		  \hline
	5 & TRANSCO & Transmission system stability  & 
		     Protection systems (millisec)	 
		     \\
		     \hline
 	6 & DISCO - Customer & Electric service & Power delivery (real-time)
 	\\
 	\cline{3-4}
 	& & Power quality  & 
		     Voltage control (hours)	 
		     \\
		     \hline
		     
 	7 & DISCO - Transportation & Special Tariff  & Time-of-Use Rate (monthly billing)
 	\\
 	\hline
 	8 & ISO - DISCO  & Power purchase  & Participation in energy markets (minutes to day-ahead)
 	\\
 	\hline
 	 9 & ISO - Aggregator  & 
 	 Power purchase, Demand response  &
 	 \begin{itemize}
 	 \item Participation in energy and ancillary service markets (minutes to day-ahead) 
 	 \item Emergency energy (minutes to hours)
 	 \end{itemize}
 	\\
 	\hline
 	 	 10 & DISCO - Aggregator  & Electricity delivery service purchase & Contract management (year)
 	\\
 	\hline
 	 	 11 & Aggregator - Transportation  & Charging service   & power delivery (real-time)
 	\\
 	\hline
 	 	 12 & Aggregator - Customer  & Flexible contracts  & Participation in energy and ancillary service markets (minutes to day-ahead)
 	\\
 	\hline
	\end{tabular}
\end{table*}

%%%%%%%%%%%%%%%%%%%%%%

In this subsection we provide an overview of the temporal division between planning and operations, as well as the spatial division between the transmission and distribution systems. 

\subsubsection*{Transmission System Planning} \label{sec:trans_planning}

Transmission systems in the US are planned on a regional basis with the aim of meeting future demand and maintain grid reliability as the fleet of generating resources and their locations continues to evolve. In some areas Regional Transmission Organizations (RTOs) conduct the transmission planning process. Transmission owners are predominantly compensated for their investments in the transmission network via cost-based rates. Building transmission infrastructure is a complicated and slow process, with concerns being raised that the process may not be able to accommodate the needs of large-scale renewable integration. The best renewable resource areas are often in more remote locations where the electric transmission infrastructure is weak \cite{ESIG2021}.


\subsubsection*{Transmission System Operations} \label{sec:trans_ops}
The ISO is responsible for running the wholesale market into which GENCOs and DISCOs submit their offers and bids for power. In turn the GENCOs are responsible for procuring fuel (Loop 1 in Figure \ref{fig:old_loops}) for fulfilling the schedules determined by the ISO. The ISO has to take into consideration several other issues including how to ensure reliable delivery of power in the event of disruptions aka contingencies. The ISO also has a number of other functions needed for the reliable operation of the transmission level grid, including administering products for energy, ancillary services, capacity and financial transmission rights. The ISO also coordinates with the TRANSCOs on transmission system outage scheduling and planning. While the TRANSCOs are responsible for maintenance of transmission equipment (Loop 5). In non-ISO areas the vertically integrated electric companies continue to be responsible for both transmission and distribution system operations.

\subsubsection*{Distribution System Planning} \label{sec:IRP}
Today typically the DISCO owns the distribution grid and is responsible for planning and operations to maintain its reliability. It is responsible for procuring power to supply the demand of all its customers. Some DISCOs generate their own power (particularly in the vertically integrated paradigm), or purchase power from other entities via power purchase agreements, or from a wholesale electricity market. 

Utilities undertake a comprehensive process to develop Integrated Resource Plans (IRPs) to ensure that there is an adequate portfolio of supply-side and demand-side resources to meet the peak demand and energy needs of their customers at least cost, typically over a 10-20 year planning horizon \cite{wilson2013best}. Resource planning requirements differ from state to state. The plans account for variety of risks including load growth, fuel prices, fuel diversity and emissions, and require the involvement of state public utility commissions (PUCs) along with other stakeholders. Thus societal choices are introduced into the planning of the grid infrastructure, for example, through state renewable portfolio standards.

\subsubsection*{Distribution System Operations} \label{sec:dist_ops}

Many DISCOs use Supervisory Control and Data Acquisition (SCADA) systems for ensuring the correct operation of substation equipment, through data acquisition, monitoring and control of the distribution system. SCADA combines hardware, software and communications to monitor various equipment, send control signals and perform key operations such as voltage control, load balancing, power quality monitoring, fault protection etc.
The first layer in this is the hardware that actuates and monitors the system conditions, including reclosers, capacitor controls, voltage regulators, fault current indicators etc. The second layer does the data collection, communication and control through remote terminal units (RTUs) and intelligent electronic devices (IEDs). The third layer is responsible for communications with the host platform typically in the control center. The fourth layer is the software platform that integrates the multiple data streams, analyses it and provides the capabilities for display and interaction to the human operators.

Today most intelligence at the distribution level is in substations with limited control and visibility downstream through devices such as reclosers, customer smart meters etc. In the future more intelligence is likely to be deployed behind the customer meters via EV software, smart thermostats, home stationary batteries etc.

%%% --------- EV charging station ----------------
The EV charging station placement is typically formulated as an optimization problem. For example, Cui \emph{et al.} formulate the problem as follows \cite{8673613}:
\begin{subequations}
    \begin{align}
        \min_{x_n, y_n \forall n \in \mathcal{N}} \quad & c(x_1,\ldots, x_n, y_i, \ldots, y_n)\\
        \text{s.t.} \quad & x_n \in \{0,1\}, y_n \in \mathbb{Z}^+ \quad \forall n\in\mathcal{N}\\
        & \sum_{n\in \mathcal{N}}s(y_n)\ge S \quad \forall n\in\mathcal{N}\\
        & f(\abs{V_n}, \delta_n, P_n, Q_n) = 0 \quad \forall n\in\mathcal{N}\\
        & \abs{I_m} \le \bar{I}_m, \quad m \in \mathcal{B}\\
        & \underline{V}_n \le \abs{V_n} \le \bar{V}_n, \quad n \in \mathcal{N}\\
        & c(x_1,\ldots, x_n, y_i, \ldots, y_n) \le \bar{c}
    \end{align}
\end{subequations}
where binary variable $x_n$ indicates if a charging station is located at node $n$ (1: yes; and 0: no); $y_n$ denotes the number of new charging spots at node $n$; $c(\cdot)$ is a cost function; sets $\mathcal{N}$ and $\mathcal{B}$ collect the indices of nodes and branches, respectively; function $s(\cdot)$ is a charging demand function; $S\in \mathbb{R}$ is the minimum power demand in the area under study; $f(\cdot)$ represents power flow equations; $\abs{V_n}$, $\delta_n$, $P_n$, and $Q_n$ denote voltage magnitude, voltage phase angle, real and reactive power injection at node $n$; $\abs{I_m}$ and $\bar{I}_m$ are current magnitude and current limit of branch $m$; $\abs{V_n}$, $\underline{V}_n$ and $\bar{V}_n$ are voltage magnitude, lower and upper limit at node $n$; and $\bar{c}$ is budget limit. The cost function includes the fix construction cost of new charging station, cost of distribution system expansion, voltage regulation cost, and so on. The approaches to approximating these costs are reported in \cite{8673613}.


Here we present one representative problem formulation of the EV charging problem proposed in \cite{6313962}. Suppose that there are $N$ EVs coordinated by an aggregator. A scheduling horizon, e.g., $24$h, can be evenly divided into $K$ time slots with the time slot length $\Delta K$. For time slot $k\in [1, 2, \ldots, K]$, the aggregator is assumed to be able to control the charging rate $w_n[k]$ of EV charger $n\in[1, 2, \ldots, M]$. Assume that the charging rate $w_n[k]$ is constant over the $k$-th time slot. Denote by $k_ {\text{start}}^{[n]}$ and $k_ {\text{end}}^{[n]}$ the starting and ending time of the $n$-th EV, respectively. The charging profile upper bound function $\bar{w}_n[k]$ is defined by \cite{6313962}
\begin{equation}
    \bar{w}_n[k] =
    \begin{cases}
         w^{[n]}_{\text{max}}, & \quad k\in[k_ {\text{start}}^{[n]}, k_ {\text{end}}^{[n]}]\\
         0, & \text{otherwise}
    \end{cases}
\end{equation}
where $w^{[n]}_{\text{max}}>0$ is the maximal charging rate of the $n$-th EV charger. In \cite{6313962}, Gan \emph{et al.} formulates the EV charging problem as follows:
\begin{subequations} \label{eq:EV_charging}
    \begin{align}
        \min_{w_1, \dots, w_M}\quad &L(w_1, \ldots, w_M) \label{eq: constrain1}\\
        \text{subject to} \quad& 0\le w_n[k] \le \bar{w}_n[k] \quad \forall n, k\\
        &\eta_n \sum_{k = 1}^K w_n[k] \Delta K = C_n(s_{\text{end}}^{[n]}-s_ {\text{start}}^{[n]}) \quad \forall n.\label{eq: constrain2}
    \end{align}
\end{subequations}

Next we present the parameters, the objective function, and the constraints in \eqref{eq:EV_charging}. Function $L(\cdot)$ is determined by the aggregator's objective. For example, it can be designed in order to minimize the line loss of the distribution system \cite{5356176}, to fill the valley of a load profile \cite{6313962}, and to establish a tradeoff between costs of energy and battery degradation \cite{ma2016efficient}. Parameters $\eta_n$, $C_n$, $s_{\text{end}}^{[n]}$, and $s_{\text{start}}^{[n]}$ are the charging efficiency, battery capacity, initial state of charge (SOC), and final SOC of EV $n$, respectively \cite{6313962}. The final SOC is specified by the EV user. Constraint \eqref{eq: constrain1} says that the charging rate of each EV cannot exceed the maximal charging rate of its charger. Constraint \eqref{eq: constrain2} suggests that each EV is required to reach its final SOC at the end of the planning horizon. In a future distribution system, an aggregator may need to coordinate thousands of EVs. As a result, solving \eqref{eq:EV_charging} will require immense amount of computation resources that may not be available in practice. In \cite{6313962}, Gan \emph{et al.} leverage computation capacity at grid edges (i.e., EV chargers), and optimization \eqref{eq:EV_charging} is solved collaboratively by the aggregator and thousands of EV charges.

$P_{\text{total}}^{\text{ref}}(t)$ by solving the following optimization problem:
\begin{subequations} \label{eq:LSE_UC}
    \begin{align}
        \min_{u_n(t)\forall n = 1, \ldots, Z} &\int_0^T \sum _{n=1}^ZP\hat{\pi}(t)u_n(t)dt\\
        \text{s.t.} \quad& u_n \in \{0, 1\}\\
        & \frac{d\theta_n(t)}{dt}=
        \alpha_n\left(\hat{\theta}_{\text{a}}(t)-\theta_n(t)\right)-\beta_n\eta P u_n(t),\\
        & \int_0^T \sum_{n = 1}^Z P u_n(t) dt = E,\\
        &\theta_n(t) \in [L_{n0}, U_{n0}],
    \end{align}
\end{subequations}
where the binary variable $u_n$ suggests the on/off status of the $n$-th AC (1 for on, and 0 for off); $\hat{\pi}(t)$ is the predicted electricity price at time $t$; $P>0$ denotes the electrical power drawn; $\eta>0$ is the AC energy efficiency coefficient; $\theta_n(t)$ denotes the indoor temperature trajectory around the $n$-th AC; the $\hat{\theta}_{\text{a}}(t)$ is the ambient temperature forecasts; $\alpha_n, \beta_n>0$ are model parameters for the $n$-th AC; $E$ is the energy budget; and $[L_{n0}, U_{n0}]$ denotes the temperature comfort range of the $n$-th customer. Solving the optimization problem \eqref{eq:LSE_UC} even for a very small-scale system, e.g., with $Z=2$, is time-consuming \cite{7742416}. To address this issue, Halder {\it{et al.}} solve the linear programming relaxation of \eqref{eq:LSE_UC}. Denote by $u_n^*(t)$ for $n=1, 2, \ldots, Z$ the solution to \eqref{eq:LSE_UC}. The reference point $P_{\text{total}}^{\text{ref}}(t)$ for the aggregated ACs is $\sum_{n=1}^Z P u_n^*(t)$. 
%% ------------- Demand Response -----------------------------
With the total power reference point for the aggregate ACs, the second layer shown in Figure \ref{fig:LSE} aims to change the setpoint $s_n(t)$ of each AC in order to drive the total power consumption $P_{\text{total}}(t)$ to track the reference point $P_{\text{total}}^{\text{ref}}(t)$ while the comfort temperature for each individual home is maintained. To this end, the aggregator first computes a command $v(t)$ via a setpoint controller (a proportional–integral–derivative controller) and broadcasts $v(t)$ to each individual AC. Each AC changes its setpoint $s_n(t)$ according to $v(t)$ and maintain the temporature trajectory $\theta_n(t)$ within the temperature comfort range of the customer. In the process above, the aggregator enables the total energy consumption to track the its optimal setpoint without measuring internal states of ACs and without satisfying customers' comfort. \prk{In this case it would be good to show the control loop involved between aggregator and customer.}







\begin{figure*}[tbp] \label{fig:old_loops}
  \centering
  \begin{minipage}[b]{1.0\linewidth}
    \centering
    \includegraphics[width=0.5\textwidth]{Fig/Old.png}
    \vspace{5mm}
    	\begin{tabular}{c|p{0.2\textwidth}|p{0.2\textwidth}|p{0.3\textwidth}}
	\hline

	\hline
	\textbf{Loop \#} & \textbf{Pair of Entities} & \textbf{Interaction} & \textbf{Control Actions (timescale)}\\
	\hline
		 1 & GENCO - Gas pipeline/marketer & Fuel supply & \begin{itemize}
		 \item Fuel reliability (real-time)
		 \item Gas purchases (day-ahead to months-ahead)
		 \end{itemize}\\
		 \hline
		 2 & GENCO - ISO & Power balance & 
        \begin{itemize}
		     \item AGC (sec/min)
		     \item Economic Dispatch (hours)
		     \item Unit Commitment (days-ahead)
		 \end{itemize}\\
		 \cline{3-4}
		 & & Capacity scheduling & Outage coordination (weeks/months)\\
		\cline{3-4}
        & & Capacity planning & Generation planning (years)\\
	\hline
	3 & ISO - TRANCO & Transmission reliability & 
	\begin{itemize}
		     \item Monitoring voltage, flows, line limits etc. (real-time)
		     \item Outage coordination (weeks/months)
		     \item Transmission line planning (years)
		 \end{itemize}\\
		 \hline
	4 & GENCO & Generator control & 
		     AVR and Governor actions (sec)
		     \\
		  \hline
	5 & TRANCO & Transmission system stability  & 
		     Protection systems (millisec)	 
		     \\
		     \hline
 	6 & DISCO - Customer & Electric service & Power delivery (real-time)
 	\\
 	\cline{3-4}
 	& & Power quality  & 
		     Voltage control (hours)	 
		     \\
		     \hline
		     
 	7 & DISCO - Transportation & Charging Services  & 
 	Power delivery (Real-time)
 	\\
 	\hline
 	8 & ISO - DISCO  & Power purchase  & Participation in energy markets (minutes to day-ahead)
 	\\
 	\hline
 	 9 & ISO - Aggregator  & 
 	 Power purchase, Demand response  &
 	 \begin{itemize}
 	 \item Participation in energy and ancillary service markets (minutes to day-ahead) 
 	 \item Emergency energy (minutes to hours)
 	 \end{itemize}
 	\\
 	\hline
 	    10 & DISCO & Distribution Network Management & Outage management (hours to days), maintenance (months) \\
 	\hline
 	 	 11 & DISCO - Aggregator  & Electricity delivery service purchase & Contract management (year)
 	\\
 	\hline
 	 	 12 & Aggregator - Transportation  & Flexible contracts   & Time-of-use rate (monthly billing)
 	\\
 	\hline
 	 	 13 & Aggregator - Customer  & Flexible contracts  & Participation in energy and ancillary service markets (minutes to day-ahead) \thuang{should this be the same with loop 12?}
 	\\
 	\hline
	\end{tabular}
  \end{minipage}
   \caption{The existing control loops in current power systems \prk{More vertical space needed between figure and table. Is Table font bigger than the font used in the paper? If so, we can reduce the table font size. Maybe we can make it a snazzy table by doing it in Excel  with noce borders, etc, and then pasting it here?}}
\end{figure*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% REVISION 

\prk{The reviewers wanted us to address the following. We should be able in our rebuttal to precisely point out a page and paragraph where we have discussed each of these explicitly. Only that will convince the Editor that we have addressed the reviewers' concerns:
\begin{enumerate}
\item Dynamic of EV Charging. We have done this.
\item Centralized vs Decentralized architectures. I am not sure if we have done this. For example DER vs centralized generation create different issues. Any others? EV charging? Etc. Can we say something stimulating? Do we need to have a specific paragraph describing the challenges of distributed vs centralized operation. 
{\color{red}{AT: I don't know whether this fully answers the concern of the reviewer, but my 2cents are:
Traditional power systems rely on a mix of centralized controls (e.g., scheduling, dispatch) and decentralized (protection relays, AVRs, Governors).
As the industry is in transition with the increase in penetration of DERs, we are likely to see some grid support services being provided by controllable resources, usually with very similar control architectures, as initially many end users will continue to depend on bulk power system for part of their power. Further, there continue to remain economics of scale e.g. large on-shore and off-shore wind farms, which could justify the need for continuing centralization. There may be fully or mostly decentralized schemes in niche cases, such as in islands and remote micro-grids. While decentralized control is generally considered faster than centralized, there may still be a need for coordination/communication. With indepedent micro-grids we may see peer-to-peer transactions with distributed intelligence to maintain grid reliability.}}

\item Event-based to Model-based. I am not sure we have dealt with this explicitly. Does he mean Data-driven vs Model driven? Or does he mean Event-Driven vs Time triggered? Maybe we scould add a paragraph. Astrom has a paper called Lebesgue samplng where he talks about the latter. \textcolor{blue}{In the response letter, we assume the ``event-based'' means ``measurement/data-driven''. In Sections III-E and III-H, we add the need of injecting data-driven approaches to grid operations.}
\item Estimating and improving System Inertia. Have we done this explicitly? Should we say something explicit somewhere on ``estimating" inertia? {\color{red}{[AT: We have added a few sentences in II-D and V-A. Should we write more?]}}
\item Interacting between Electricity and other Energy Sectors (heat/cool sectors, Hydrogen). We have done this.
\item Coordination between vectors: p2X, X2P, Energy Storage sectors, operation and control. Have we done this adequately?
\item V2G: Importance in future low-inertia systems. Have we done enough regarding this?
\item Resilience and micro-grid. We have talked about this.
\end{enumerate}
}

